H-TRIP: Exact Many-to-Many Distance Index for Multi-Robot Exploration

Frontier-based exploration systems repeatedly evaluate geodesic travel costs between robot poses and candidate viewpoints, and tour-based planners consume the full pairwise distance matrix built from them. Recomputing these matrices with one graph search per source scales with the explored map size, whereas distance caches that refresh only locally affected or newly created frontiers can retain stale costs between surviving pairs when newly discovered free space creates a global shortcut. We present H-TRIP (Hierarchical Tropical Rank-one Incremental Propagation), an exact distance index grounded in Kleene algebra over the min-plus semiring for monotonically growing occupancy grids. H-TRIP partitions the known map into a spatial hierarchy with fixed boundary ports. Each unknown-to-free revelation is decomposed into efficient rank-one min-plus edge insertions at the affected leaf, and only decreased port-to-port summaries are propagated along its ancestor chain. A shared hierarchical lift evaluates the dense many-to-many matrix of shortest distances for all active query points on the occupancy map. We prove that sequential insertions preserve exact shortest-path distances on the grid. Benchmark experiments confirm exact agreement with reference searches on fully built maps and show that dense many-to-many queries at a few dozen viewpoints are up to two orders of magnitude faster than sequential k x BFS. On exploration runs with sixteen robots, in-loop queries on the growing occupancy graph are 2.21x-8.59x faster than co-scheduled k x BFS on maps with side 256, 512, and 1024 cells.

==> figures/tab-notation.tex <==
% !TEX root = ../minplus-icra2027.tex
% Two single-column floats: a later symbol appears only after those its meaning uses.
% Included from content/03-problem.tex.
\begin{table}[t]
\caption{Notation: occupancy graph and geodesic distance matrix.
    Matrix rows state stored size.
    A later symbol uses only symbols already listed.}
\label{tab:notation}
\centering
\scriptsize
\setlength{\tabcolsep}{2.8pt}
\setlength{\arraystretch}{0.95}
\begin{tabular}{@{}l p{0.64\columnwidth}@{}}
\toprule
Symbol & Meaning \\
\midrule
\(\overline{\mathbb{R}}_{\ge 0}\) &
  Extended nonnegative reals \(\mathbb{R}_{\ge 0}\cup\{\infty\}\), the value set of geodesics and closures. \\
\(\oplus\), \(\otimes\) &
  Semiring \(\min\) and \(+\). Multiplicative identity \(0\); additive identity \(\infty\). \\
\(A\) &
  Weighted adjacency of an \(n\)-vertex graph, size \(n\times n\). \\
\(I_n\) &
  Min-plus identity, size \(n\times n\): \(0\) on the diagonal, \(\infty\) off it. \\
\(A^*\), \(D\) &
  Kleene star \(D=A^*=I_n\oplus A\oplus\cdots\oplus A^{\otimes(n-1)}\), size \(n\times n\): shortest-path lengths, \(\infty\) if unreachable. \\
\(B\) &
  Rank-one perturbation of \(A\), size \(n\times n\). An opening is \((A\oplus B)^*\). \\
\midrule
\(\mathcal{W}\) &
  Planar workspace \(\subset\mathbb{R}^2\). \\
\(M\) &
  Occupancy grid on \(\mathcal{W}\). Cells are \(\texttt{unknown}\), \(\texttt{free}\), or \(\texttt{obstacle}\). \\
\(\tau\) &
  Discrete index of successive occupancy graphs. \\
\(G_\tau=(V_\tau,E_\tau)\) &
  Free-cell graph at index \(\tau\). Default \(E_\tau\): unit \(4\)-adjacent edges. \\
\(d_{G_\tau}(u,v)\) &
  Shortest-path length on \(G_\tau\); \(\infty\) if unreachable. \\
\(\Delta V\) &
  Newly free cells of an opening, so \(V_{\tau+1}=V_\tau\cup\Delta V\). \\
\(\Delta E\) &
  Newly finite incident edges of an opening, so \(E_{\tau+1}=E_\tau\cup\Delta E\). \\
\midrule
\(N\) &
  Number of robots. \(SE(2)\) pose; \(D_\tau\) uses planar position \(r_i\), snapped to a free cell \(\tilde{r}_i\) of \(G_\tau\). \\
\(\mathcal{F}_\tau=\{F_1,\dots,F_K\}\) &
  Frontier clusters: connected free cells adjacent to \(\texttt{unknown}\). \\
\(K\) &
  Cluster count \(K=|\mathcal{F}_\tau|\). \\
\(m(F_i)\) &
  Medoid cell of cluster \(F_i\) on \(G_\tau\). \\
\(P_\tau\) &
  Viewpoint list \((\tilde{r}_1,\dots,\tilde{r}_N,\,m(F_1),\dots,m(F_K))\). \\
\(k\) &
  \(|P_\tau|=N+K\). \\
\(D_\tau\) &
  Geodesic distance matrix, size \(k\times k\), \((D_\tau)_{ij}=d_{G_\tau}(P_{\tau,i},P_{\tau,j})\). Symmetric; diagonal \(0\). \\
\(D_{\tau,RR}\) &
  Robot--robot block of \(D_\tau\), size \(N\times N\). \\
\(D_{\tau,RF}=D_{\tau,FR}^{\top}\) &
  Robot--frontier block of \(D_\tau\), size \(N\times K\). Assignment reads this block. \\
\(D_{\tau,FF}\) &
  Frontier--frontier block of \(D_\tau\), size \(K\times K\). Open tours read this block. \\
\(\widehat{D}_{\tau+1}\) &
  New-cluster-only cache, size \(k\times k\): persisting coordinates keep \((D_\tau)_{ij}\). \\
\(\mathcal{F}_{\mathrm{surv}}\) &
  Clusters whose medoids occupy the same cells in \(P_\tau\) and \(P_{\tau+1}\). \\
\(p_i,p_j\) &
  A surviving pair: same cells in \(P_\tau\) and \(P_{\tau+1}\). \\
\(\mathcal{I}\) &
  Index: map \(\mathcal{I}:V_\tau^{k}\to\Rmin^{k\times k}\). After an opening, \(\mathcal{I}(P_{\tau+1})\) equals \(D_{\tau+1}\). \\
\(K_{\max}\) &
  Cap on clusters in \(P_\tau\), so \(K\le K_{\max}\). \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\caption{Notation: hierarchy, closures, update, and query.
    Continues Table~\ref{tab:notation}.
    Matrix rows state stored size.}
\label{tab:notation_oracle}
\centering
\scriptsize
\setlength{\tabcolsep}{2.8pt}
\setlength{\arraystretch}{0.95}
\begin{tabular}{@{}l p{0.64\columnwidth}@{}}
\toprule
Symbol & Meaning \\
\midrule
\(b\) &
  Leaf side in cells, an integer \(b\ge 2\). Experiments use \(b=16\), or \(b=32\) on Boston \(1024\). \\
\(g\) &
  Tile aggregation degree, an integer \(g\ge 2\). Each internal node has \(g^2\) children. \\
\(S\) &
  Root side \(S=bg^{H}\ge n\) for an \(n\times n\) square grid \(M\). \\
\(H\) &
  Depth \(H=\lceil\log_g(n/b)\rceil\) from \(n\), \(b\), and \(g\). \\
\(T\), \(U\) &
  Base tile of side \(b\); super-tile parent. \\
\(b_\ell\) &
  Side of a level-\(\ell\) tile, \(b_\ell=bg^{\ell}\), so \(b_0=b\). \\
\(B_T\) &
  Fixed boundary cells of \(T\): \(4b_\ell-4\) perimeter cells, independent of passability. \\
\(\Omega_T\) &
  Local index set of the stored closure of \(T\). Base: the \(b^2\) geometric cells. Super-tile: \(\Omega_U=\bigsqcup_Q\varphi_{Q\to U}(B_Q)=V_U\). \\
\(A_T\), \(C_T=A_T^*\) &
  Tile-local adjacency and metric closure, size \(|\Omega_T|\times|\Omega_T|\). An entry of \(C_T\) may exceed the global geodesic on \(G_\tau\). \\
\(S_T\) &
  Boundary summary \(S_T=C_T|_{B_T\times B_T}\), the Cartesian product of boundary indices, size \((4b-4)\times(4b-4)\) at a base tile. \\
\(V_U\) &
  Vertex set of \(\Gamma_U\), equal to \(\Omega_U\). For leaf children of side \(b\), \(|V_U|=g^2(4b-4)\). \\
\(\varphi_{Q\to U}\) &
  Fixed index mapping from a child tile \(Q\) into \(\Omega_U\); image \(\overline{B}_Q^{U}\). \\
\(C_U\) &
  Interface closure \(C_U=A_U^*\), size \(|\Omega_U|\times|\Omega_U|\). \\
\(\Gamma_U\) &
  Condensed interface graph of super-tile \(U\). \\
\(B_U\), \(S_U\) &
  Exterior boundary cells \(B_U\subset V_U\); \(S_U=C_U|_{B_U\times B_U}\). \\
\midrule
\(c\) &
  Newly free cell in leaf \(T_{\mathrm{leaf}}\). \\
\(E_{\mathrm{intra}}\), \(E_{\mathrm{seam}}\) &
  New intra-leaf edges at \(c\); new inter-tile seam edges at \(c\). \\
\(n\), \(m_T\) &
  Workspace side of square \(M\); \(m_T=|\Delta V\cap T|\) newly free cells of the opening in \(T\). Leaf update \(O(m_T b^4)\). \\
\(\Pi\), \(\Pi_U\) &
  Endpoints of \(F_T\) and of \(F_U\). \\
\(\Delta S_T\), \(\Delta S_U\) &
  Strictly decreased entries of \(S_T\) and of \(S_U\), with updated values. \\
\(F_T\), \(F_U\) &
  Decreased undirected edges at a base tile and at a parent interface. \\
\midrule
\(s\), \(t\) &
  Query source and target in \(V_\tau\). \\
\(T_s^{(\ell)}\), \(T_t^{(\ell)}\) &
  Level-\(\ell\) ancestors of the leaves containing \(s\) and \(t\). \\
\(x_s^{(\ell)}\), \(y_t^{(\ell)}\) &
  Source and target attachments. Leaf: \(x_s^{(0)}=C_{T_s}(s,B_{T_s})\). \\
\(\chi_U(s)\), \(Q_s\), \(Q_t\) &
  Child of \(U\) containing \(s\); \(Q_s=\chi_U(s)\), \(Q_t=\chi_U(t)\). \\
\(d_U(s,t)\) &
  Meet \(x_{s\to Q_s}\otimes C_U|_{\overline{B}_{Q_s}^{U}\times\overline{B}_{Q_t}^{U}}\otimes y_{Q_t\to t}\). \\
\(d(s,t)\) &
  \(\min\) over enclosing ancestors of \(d_U(s,t)\), and \(C_{T_s}(s,t)\) if \(T_s=T_t\). Equals \(d_{G_\tau}(s,t)\). \\
\(|B_Q|\), \(|B_{\max}|\) &
  Boundary count of a child that contains query viewpoints; \(|B_{\max}|=\max_{\ell}|B_{T_s^{(\ell)}}|\). \\
\(k_{\mathrm{hybrid}}\) &
  BFS-fallback threshold. Timed H-TRIP uses \(0\) (Section~\ref{sec:eval_setup}). \\
\(s\) &
  Explorer scale \(s\in\{1,2,4\}\) at \(5\,\mathrm{cm}\) per unscaled cell. Unused on query-only native maps. \\
\(\texttt{INF}\) &
  \(\texttt{uint16}\) sentinel \(60000\). Theorems are identities over \(\overline{\mathbb{R}}_{\ge 0}\). \\
\bottomrule
\end{tabular}
\end{table}

